New Insights on Interstellar Gas-Phase Iron

In this paper, we report on the gas-phase abundance of singly-ionized iron (Fe II) for 51 lines of sight, using data from the Far Ultraviolet Spectroscopic Explorer (FUSE). Fe II column densities are derived by measuring the equivalent widths of several ultraviolet absorption lines and subsequently fitting those to a curve of growth. Our derivation of Fe II column densities and abundances creates the largest sample of iron abundances in moderately- to highly-reddened lines of sight explored with FUSE, lines of sight that are on average more reddened than lines of sight in previous Copernicus studies. We present three major results. First, we observe the well-established correlation between iron depletion and <n_H> and also find trends between iron depletion and other line of sight parameters (e.g. f(H_2), E_(B-V), and A_V), and examine the significance of these trends. Of note, a few of our lines of sight probe larger densities than previously explored and we do not see significantly enhanced depletion effects. Second, we present two detections of an extremely weak Fe II line at 1901.773 A in the archival STIS spectra of two lines of sight (HD 24534 and HD 93222). We compare these detections to the column densities derived through FUSE spectra and comment on the line's f-value and utility for future studies of Fe II. Lastly, we present strong anecdotal evidence that the Fe II f-values derived empirically through FUSE data are more accurate than previous values that have been theoretically calculated, with the probable exception of f_1112.

==> macros.tex <==
\newtheorem{theorem}{Theorem}


\newcommand{\diff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diffr}[1]{\diff{#1}{r}}
\newcommand{\diffth}[1]{\diff{#1}{\theta}}
\newcommand{\diffz}[1]{\diff{#1}{z}}

\newcommand{\vth}{V_{\theta}}

\newcommand{\twochoices}[2]{\left\{ \begin{array}{lcc}
        \displaystyle #1 \\ \vspace{-10pt} \\
        \displaystyle #2 \end{array} \right. } %}

\newcommand{\threechoices}[3]{\left\{ \begin{array}{lcc}
        #1 \\ #2 \\ #3 \end{array} \right. }    %}

\newcommand{\fourchoices}[4]{\left\{ \begin{array}{lcc}
        #1 \\ #2 \\ #3 \\ #4 \end{array} \right. }      %}

\newcommand{\twovec}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\threevec}[3]{\left(\begin{array}{c} #1 \\ #2 \\ #3 \end{array}\right)}
\newcommand{\twomatrix}[4]{\left(\begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array}\right)}

% Solar commands
\newcommand{\mdot}{{\dot{\rm M}}}
\newcommand{\msun}{{~{\rm M}_\odot}}
\newcommand{\msunperyr}{{\msun {\rm yr}^{-1}}}
% Unit commands
\newcommand{\kmpers}{{{\rm \; km\;s}^{-1}}}
\newcommand{\ppm}{{\rm \; ppm}}
\newcommand{\percc}{{\rm \; cm}^{-3}}
\newcommand{\dex}{{\rm \; dex}}
\newcommand{\magnitude}{{\rm \; mag}}
% Abundance commands
\newcommand{\logOH}{{\log{{\rm(O/H)}}}}
\newcommand{\logNH}{{\log{{\rm(N/H)}}}}
\newcommand{\logFeH}{{\log{{\rm(Fe/H)}}}}
\newcommand{\logFeIIH}{{\log{{\rm(Fe \; II/H)}}}}
\newcommand{\logMgH}{{\log{{\rm(Mg/H)}}}}
\newcommand{\logMgIIH}{{\log{{\rm(Mg \; II/H)}}}}
\newcommand{\logSiH}{{\log{{\rm(Si/H)}}}}
\newcommand{\logSiIIH}{{\log{{\rm(Si \; II/H)}}}}
\newcommand{\Htot}{{\rm H_{tot}}}
\newcommand{\OH}{{\rm O/H}}
\newcommand{\NH}{{\rm N/H}}
\newcommand{\FeH}{{\rm Fe/H}}
\newcommand{\MgH}{{\rm Mg/H}}
\newcommand{\SiH}{{\rm Si/H}}
\newcommand{\OHsolar}{{\rm(O/H)}_{\odot}}
\newcommand{\OHdust}{{\rm O_{dust}/H}}
%Column density commands
\newcommand{\NHI}{{N{\rm(H \; I)}}}
\newcommand{\NOI}{{N{\rm(O \; I)}}}
\newcommand{\NNI}{{N{\rm(N \; I)}}}
\newcommand{\NHmol}{{N\rm(H_{2})}}
\newcommand{\NFe}{{N{\rm(Fe)}}}
\newcommand{\NFeII}{{N{\rm(Fe \; II)}}}
\newcommand{\logFeII}{{\log{N{\rm(Fe \; II)}}}}
\newcommand{\NMg}{{N{\rm(Mg)}}}
\newcommand{\NMgII}{{N{\rm(Mg \; II)}}}
\newcommand{\logMgII}{{\log{N{\rm(Mg \; II)}}}}
\newcommand{\NSi}{{N{\rm(Mg)}}}
\newcommand{\NSiII}{{N{\rm(Si \; II)}}}
\newcommand{\logSiII}{{\log{N{\rm(Si \; II)}}}}
\newcommand{\logHI}{{\log{\NHI}}}
\newcommand{\logHmol}{{\log{\NHmol}}}
\newcommand{\logHtot}{{\log{\NHtot}}}
\newcommand{\logOI}{{\log{N\rm(O \; I)}}}
\newcommand{\logNI}{{\log{N\rm(N \; I)}}}
\newcommand{\NHtot}{{N{\rm(H_{tot})}}}
% Molecular commands
\newcommand{\Hmol}{{\rm H_{2}}}
\newcommand{\Nmol}{{\rm N_{2}}}
% Line of sight parameter commands
\newcommand{\nH}{{\rm{n_{H}}}}
%\newcommand{\nHavg}{{\langle \rm{n_{H}} \rangle}}
\newcommand{\nHavg}{{< \! \! \rm{n_{H}} \! \! >}}
\newcommand{\nHvol}{{\rm n_{H}}}
\newcommand{\lognh}{{\log{\nH}}}
\newcommand{\lognHavg}{{\log{\nHavg}}}
\newcommand{\lognha}{{\log{\nHavg}}}
\newcommand{\fHmol}{{f\rm(H_{2})}}
% Other commands
\newcommand{\eqw}{{W_{\lambda}}}
\newcommand{\av}{{A_V}}
\newcommand{\alamb}{{A_{\lambda}}}
\newcommand{\ebv}{{E_{B-V}}}
\newcommand{\elambv}{{E_{\lambda-V}}}
\newcommand{\avdist}{{\av / r}}
\newcommand{\ebvdist}{{\ebv / r}}
\newcommand{\rv}{{R_V}}
\newcommand{\nelec}{{\rm n_{e}}}
